Passport: Improving Automated Formal Verification Using Identifiers

Formally verifying system properties is one of the most effective ways of improving system quality, but its high manual effort requirements often render it prohibitively expensive. Tools that automate formal verification, by learning from proof corpora to suggest proofs, have just begun to show their promise. These tools are effective because of the richness of the data the proof corpora contain. This richness comes from the stylistic conventions followed by communities of proof developers, together with the logical systems beneath proof assistants. However, this richness remains underexploited, with most work thus far focusing on architecture rather than making the most of the proof data. In this paper, we develop Passport, a fully-automated proof-synthesis tool that systematically explores how to most effectively exploit one aspect of that proof data: identifiers. Passport enriches a predictive Coq model with three new encoding mechanisms for identifiers: category vocabulary indexing, subword sequence modeling, and path elaboration. We compare Passport to three existing base tools which Passport can enhance: ASTactic, Tac, and Tok. In head-to-head comparisons, Passport automatically proves 29% more theorems than the best-performing of these base tools. Combining the three Passport-enhanced tools automatically proves 38% more theorems than the three base tools together, without Passport's enhancements. Finally, together, these base tools and Passport-enhanced tools prove 45% more theorems than the combined base tools without Passport's enhancements. Overall, our findings suggest that modeling identifiers can play a significant role in improving proof synthesis, leading to higher-quality software.

==> Makefile <==

FIGS=fig/main-eval-results.pdf fig/individual-techs.pdf fig/bpe-techs.pdf \
     fig/bpe-merges.pdf fig/global-vsize.pdf fig/local-vsize.pdf \
     fig/path-vsize.pdf fig/constructor-vsize.pdf fig/path-techs.pdf

all: main.pdf

main.pdf: $(wildcard *.tex) $(FIGS)
	latexmk -pdf main.tex

CoverLetter.pdf: CoverLetter.tex
	latexmk -pdf $<
clean:
	rm -f *.aux *.bbl *.blg *.fdb_latexmk *.fls *.log *.pdf

fig/main-eval-results.pdf: fig/main-eval-results.gp fig/main_results_them.dat fig/main_results_us.dat
	gnuplot $<

fig/individual-techs.pdf: fig/individual-techs.gp fig/individual-techs-us.dat fig/individual-techs-them.dat
	gnuplot $<

fig/bpe-techs.pdf: fig/bpe-techs.gp fig/individual-techs-us.dat
	gnuplot $<

fig/bpe-merges.pdf: fig/bpe-merges.gp fig/bpe-merges.dat
	gnuplot $<

fig/global-vsize.pdf: fig/global-vsize.gp fig/global-vsize.dat
	gnuplot $<

fig/local-vsize.pdf: fig/local-vsize.gp fig/local-vsize.dat
	gnuplot $<

fig/path-vsize.pdf: fig/path-vsize.gp fig/path-vsize.dat
	gnuplot $<

fig/constructor-vsize.pdf: fig/constructor-vsize.gp fig/constructor-vsize.dat
	gnuplot $<

fig/path-techs.pdf: fig/path-techs.gp fig/path-techs.dat
	gnuplot $<

